DIVeR: Real-time and Accurate Neural Radiance Fields with Deterministic Integration for Volume Rendering

DIVeR builds on the key ideas of NeRF and its variants -- density models and volume rendering -- to learn 3D object models that can be rendered realistically from small numbers of images. In contrast to all previous NeRF methods, DIVeR uses deterministic rather than stochastic estimates of the volume rendering integral. DIVeR's representation is a voxel based field of features. To compute the volume rendering integral, a ray is broken into intervals, one per voxel; components of the volume rendering integral are estimated from the features for each interval using an MLP, and the components are aggregated. As a result, DIVeR can render thin translucent structures that are missed by other integrators. Furthermore, DIVeR's representation has semantics that is relatively exposed compared to other such methods -- moving feature vectors around in the voxel space results in natural edits. Extensive qualitative and quantitative comparisons to current state-of-the-art methods show that DIVeR produces models that (1) render at or above state-of-the-art quality, (2) are very small without being baked, (3) render very fast without being baked, and (4) can be edited in natural ways.

==> equations/linear_basis.tex <==
\begin{gather}
    %g(\mathbf{r}(t)) \sim \mathbf{w}^\top \mathbf{f}(\mathbf{r}(t)) \\
    %\int_a^b g(\mathbf{r}(t)) \sim \mathbf{w}^\top \int_a^b\mathbf{f}(\mathbf{r}(t))dt\\
    \begin{gathered}
    \int_a^b g(t) \sim \mathbf{w}^\top \int_a^b\mathbf{f}(\mathbf{r}(t))dt\\
    \text{where}  \int_a^b\mathbf{f}(\mathbf{r}(t))dt = \\ 
    (\int_a^b f_C(\mathbf{r}(t))dt,\ldots,\int_a^b f_1(\mathbf{r}(t))dt)
    \label{eq:linear-basis}
    \end{gathered}
\end{gather}

==> equations/mlp_basis_integration.tex <==
\begin{gather}
    \int_a^b g(\mathbf{r}(t)) dt \sim \text{MLP}_{\mathbf{w}}(\int_a^b \mathbf{f}(\mathbf{r}(t))dt)\\
    \begin{gathered}
    \text{where} \int_a^b \mathbf{f}(\mathbf{r}(t)dt)=\\
    (\int_a^b f_1(\mathbf{r}(t))dt,\ldots, \int_a^b f_C(\mathbf{r}(t))dt)
    \end{gathered}
\end{gather}

==> equations/vre_approx.tex <==
\begin{equation}
    \alpha_i \mathbf{c}_i \sim
    \int_{t^\text{i}_i}^{t^\text{o}_i} e^{-\int_{t^\text{i}_i}^t \sigma(\mathbf{r}(\tau))d\tau}
    \mathbf{c}(\mathbf{r}(t),\mathbf{d})dt
\end{equation}

==> figures/architecture-daf.tex <==
\begin{figure}[t]
   \centering
   \resizebox{0.6\columnwidth}{!}{
   \begin{tabular}{c}
        \includegraphics[width=0.7\linewidth]{images/decoder64.png}\\
        \ours64\\
        \\
        \includegraphics[width=0.7\linewidth]{images/decoder32.png}\\
        \ours32
   \end{tabular}
   }
   \caption{\textbf{Decoder architectures:} the decoder takes $\mathbf{f}(\vect{x})$ integrated along an interval 
     together with positionally encoded view direction, and reports density and color for that interval.  Using a small MLP
     helps render time.       \ours64 has around
8K parameters; \ours32 has around 4k parameters.}
\label{fig:architecture}
\end{figure}


==> figures/architecture_ablation2.tex <==
\begin{figure}[t]
   \centering
   \setlength\tabcolsep{1.0pt}
   \begin{tabular}{cc}
        \includegraphics[width=0.45\linewidth]{images/chair_25650.png}&
        \includegraphics[width=0.45\linewidth]{images/chair_3250.png}\\
        \ours64$,N=256$& 
        \ours32$,N=256$\\
        \includegraphics[width=0.45\linewidth]{images/chair_12850.png}&
        \includegraphics[width=0.45\linewidth]{images/chair_gt50.png}\\
        \ours64$,N=128$& 
        Ground Truth\\
   \end{tabular}
    \caption{\textbf{Qualitative comparison of different architectures}. Larger voxel grid and decoder MLP tend to give better detail of textures on the chair.}
\label{fig:architecture-alb}
\end{figure}

==> figures/pipeline-daf.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/pipeline2.png}
    \caption{\textbf{Rendering pipeline overview.} To render a ray, we
      first find its intersection with voxels. For each voxel, the
      intersection feature at entry (resp. exit) is computed as a
      trilinear interpolate.  This yields a linear function along the
      ray (equivalently, the voxel represents a trilinear feature
      function of its vertex features).  We integrate the linear
      function along the interval within the voxel, passing the result
      to an MLP that decodes to color and alpha values for the voxel. We
      obtain the final integral estimate for the ray by accumulating
      color and alpha values along the ray.}
    \label{fig:pipeline}
\end{figure*}


==> figures/training_ablation.tex <==
\begin{figure}[t]
   \centering
   \setlength\tabcolsep{1.0pt}
   \begin{tabular}{cc}
        \includegraphics[width=0.45\linewidth]{images/lego_train_impexp.png}&
        \includegraphics[width=0.45\linewidth]{images/lego_train_imp.png}\\
        Im-Ex& 
        Im\\
        \includegraphics[width=0.45\linewidth]{images/lego_train_exp.png}&
        \includegraphics[width=0.45\linewidth]{images/lego_train_gt.png}\\
        Ex& 
        Ground Truth\\
   \end{tabular}
    \caption{\textbf{Qualitative comparison on training strategies}. Explicit model fails to model the reflection and produces glossy artifacts. While implicit and implicit-explicit model are perceptually same, implicit model has slightly worse PSNR.}
\label{fig:training-abl}
\end{figure}

